Asking and Answering Questions to Evaluate the Factual Consistency of Summaries

Practical applications of abstractive summarization models are limited by frequent factual inconsistencies with respect to their input. Existing automatic evaluation metrics for summarization are largely insensitive to such errors. We propose an automatic evaluation protocol called QAGS (pronounced "kags") that is designed to identify factual inconsistencies in a generated summary. QAGS is based on the intuition that if we ask questions about a summary and its source, we will receive similar answers if the summary is factually consistent with the source. To evaluate QAGS, we collect human judgments of factual consistency on model-generated summaries for the CNN/DailyMail (Hermann et al., 2015) and XSUM (Narayan et al., 2018) summarization datasets. QAGS has substantially higher correlations with these judgments than other automatic evaluation metrics. Also, QAGS offers a natural form of interpretability: The answers and questions generated while computing QAGS indicate which tokens of a summary are inconsistent and why. We believe QAGS is a promising tool in automatically generating usable and factually consistent text.

==> tables/ablation-qg-genre.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{lc@{/}cc@{/}c}
        \toprule
        Metric & \multicolumn{2}{c}{CNN/DM} & \multicolumn{2}{c}{XSUM} \\
        \midrule
        QAGS$_\text{NewsQA}$ & 40.94 & 38.33 & \textbf{16.61} & \textbf{16.25} \\
        QAGS$_\text{SQuAD}$ & \textbf{48.22} & \textbf{43.41} & 16.18 & 14.77 \\
        \bottomrule
    \end{tabular}
    \caption{Summary-level Pearson/Spearman correlation coefficients between various automatic metrics and human judgments of correctness for summarization datasets. *, ** denote significance at $p < 0.01, 0.001$ respectively.}
    \label{tab:ablations-genre}
\end{table}



==> tables/ablations.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{lllc@{/}cc@{/}c}
        \toprule
        QG genre & QA model & \#  & \multicolumn{2}{c}{CNN/DM} & \multicolumn{2}{c}{XSUM} \\
        \midrule
        NewsQA & \texttt{bert-large} & 20 & 40.94 & 38.33 & \textbf{16.61} & \textbf{16.25} \\
        \midrule

        SQuAD & \texttt{bert-large} & 20 & 40.94 & 38.33 & \textbf{16.61} & \textbf{16.25} \\
        \midrule

        NewsQA & \texttt{bert-base} & 20 & 40.94 & 38.33 & \textbf{16.61} & \textbf{16.25} \\
        NewsQA & \texttt{bert-large-wwm} & 20 & 40.94 & 38.33 & \textbf{16.61} & \textbf{16.25} \\
        \midrule

        NewsQA & \texttt{bert-large} & 5 & 40.94 & 38.33 & \textbf{16.61} & \textbf{16.25} \\
        NewsQA & \texttt{bert-large} & 10 & 40.94 & 38.33 & \textbf{16.61} & \textbf{16.25} \\
        NewsQA & \texttt{bert-large} & 30 & 40.94 & 38.33 & \textbf{16.61} & \textbf{16.25} \\
        NewsQA & \texttt{bert-large} & 50 & 40.94 & 38.33 & \textbf{16.61} & \textbf{16.25} \\
        \bottomrule
    \end{tabular}
    \caption{Summary-level Pearson/Spearman correlation coefficients between various automatic metrics and human judgments of correctness for summarization datasets. *, ** denote significance at $p < 0.01, 0.001$ respectively.}
    \label{tab:ablations}
\end{table}

==> tables/algorithm.tex <==
\begin{algorithm}[t]
\SetAlgoLined
\DontPrintSemicolon
\textbf{Inputs}: source $X$, summary $Y$, number of questions $K$\;
score $\leftarrow 0$\;
$Q = \{q_i\}_{i=1}^K \leftarrow \textsc{GetQuestions}(Y, K) $\;
\For{\upshape $q_i$ in $Q$}{
    $a_x \leftarrow \textsc{GetAnswer}(q_i, X)$\;
    $a_y \leftarrow \textsc{GetAnswer}(q_i, Y)$\;
    %$a_x \leftarrow \argmax p(A|X, q_i)$\;
    %$a_y \leftarrow \argmax p(A|Y, q_i)$\;
    score $ \leftarrow \text{score} + D(a_x, a_y)$\;

}
\Return{\upshape score / $K$}
\caption{QAGS score computation. 
%\textsc{GetQuestions} is a function, usually parameterized by a neural network, that takes in a text, and a integer $K$ and returns $K$ questions based on the inputted text. \textsc{GetAnswer} is a function that takes in a text question and a context, and returns an answer to the question using the context.
}
\label{fig:algorithm}
\end{algorithm}


==> tables/qags-examples-2col.tex <==
\begin{table*}[t]
    \centering
    %\begin{tabular}{p{\linewidth}}%{\linewidth}{X}
    \begin{tabularx}{\linewidth}{XX}
        \toprule
        
        \thead{\textbf{Article:} On Friday, 28-year-old Usman Khan stabbed reportedly several people at Fishmongers' Hall in London with a large knife, then fled up London Bridge. Members of the public confronted him; one man sprayed Khan with a fire extinguisher, others struck him with their fists and took his knife, and another, a Polish chef named Łukasz, harried him with a five-foot narwhal tusk. [\dots] \\
        \textbf{Summary:} On Friday afternoon , a man named Faisal Khan entered a Cambridge University building and started attacking people with a knife and a fire extinguisher .} &
        
        \thead{\textbf{Question :} Who did Faisal Khan attack ? \\
        \textbf{Article answer:} {\color{red} several people} \quad \textbf{Summary answer:} {\color{red} people}} \\
        
        %\textbf{Question:} What did the attacker have ? \\
        %\textbf{Article answer:} {\color{red} a large knife} \quad \textbf{Summary answer:} {\color{red} a knife and a fire extinguisher} \\
        
        %\textbf{Question:} When did the attack take place ? \\
        %\textbf{Article answer:} {\color{red} Friday} \quad \textbf{Summary answer:} {\color{red} Friday afternoon} \\
        
        %\textbf{Question:} What is the attacker's name ? \\
        %\textbf{Article answer:} {\color{red} Usman Khan} \quad \textbf{Summary answer:} {\color{red} Faisal Khan} \\       
        
        %\textbf{Question:} Where did the attack take place ? \\
        %\textbf{Article answer:} {\color{red} Fishmongers' Hall} \quad %\textbf{Summary answer:} {\color{red} Cambridge University building} \\ }

        \midrule
        
        %\textbf{Article: } In findings published on Wednesday in the journal PLOS ONE, an international team of scientists report ancient Egyptians captured sacred ibises (Threskiornis aethiopicus) from the wild for use in ritual sacrifice rather than domesticating the birds. [\dots] The team collected DNA samples from mummified birds collected from six separate catacombs including sites at Abydos, Saqqara, and Tuna el-Gebel with permission from the Egyptian Ministry of State for Antiquity, and several museums offered to send tissue samples from the mummified ibises in their collections. They were able to extract complete mitochondrial DNA sequences from fourteen. These they compared to those of 26 modern ibises from different parts of Africa — ibises of this species disappeared from Egypt itself during modern times. They found the DNA sequences from the ancient birds to be relatively diverse. [\dots] \\
        %\textbf{Summary:} Archaeologists have used DNA samples from ancient ibis birds to determine whether the birds were domesticated or sacrificed in ancient Egypt \\
        
        %\textbf{Question}: Archaeologists have used what to determine whether the birds were domesticated ? \\
        %\textbf{Article Answer}: hatchery structures \quad
        %\textbf{Summary Answer}: DNA samples \\
%
        %\textbf{Question}: Archaeologists have used DNA samples from what ? \\
        %\textbf{Article Answer}: mummified birds collected from six separate catacombs \quad 
        %\textbf{Summary Answer}: ancient ibis birds \\
        %
        %\textbf{Question:} Who used DNA samples to determine whether the birds were domesticated ? \\
        %\textbf{Article Answer:} [NO ANSWER] \quad
        %\textbf{Summary Answer:} Archaeologists \\
        %
        %\textbf{Question:} What are archeologists using to determine whether the birds were domesticated ? \\
        %\textbf{Article Answer:} DNA samples \quad
        %\textbf{Summary Answer:}: DNA samples \\
%
        %\textbf{Question:} Where were the birds found? \\
        %\textbf{Article Answer:} six separate catacombs \quad
        %\textbf{Summary Answer:} ancient Egypt \\
        
        \bottomrule
    %\end{tabular}
    \end{tabularx}
    \caption{Examples of the intermediate questions and answers generated when computing QAGS on news articles, along with the relevant portions of the original article and summary. The questions generated are overwhelmingly human readable and on-topic. The answers indicate which tokens in the summary are factually consistent or inconsistent.}
    \label{tab:examples}
\end{table*}

==> tables/reranking.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lc}
        \toprule
        Model/Metric & \% \\
        \midrule
        w/o reranking & \\
        w/ QAGS reranking & \\
        \bottomrule
    \end{tabular}
    \caption{}
    \label{tab:rerank}
\end{table}

==> tables/system-corr.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{ccc}
        \toprule
        Metric & CNN/DM & XSUM \\
        \midrule
        Perplexity & & \\
        ROUGE & & \\
        METEOR & & \\
        QAGS (EM) & & \\
        QAGS (F1) & & \\
        \bottomrule
    \end{tabular}
    \caption{System-level Pearson/Spearman correlation coefficients between various automatic metrics and human judgments of correctness for summarization datasets.}
    \label{tab:system-correlations}
\end{table}
